Interpretable User Satisfaction Estimation for Conversational Systems with Large Language Models

Accurate and interpretable user satisfaction estimation (USE) is critical for understanding, evaluating, and continuously improving conversational systems. Users express their satisfaction or dissatisfaction with diverse conversational patterns in both general-purpose (ChatGPT and Bing Copilot) and task-oriented (customer service chatbot) conversational systems. Existing approaches based on featurized ML models or text embeddings fall short in extracting generalizable patterns and are hard to interpret. In this work, we show that LLMs can extract interpretable signals of user satisfaction from their natural language utterances more effectively than embedding-based approaches. Moreover, an LLM can be tailored for USE via an iterative prompting framework using supervision from labeled examples. The resulting method, Supervised Prompting for User satisfaction Rubrics (SPUR), not only has higher accuracy but is more interpretable as it scores user satisfaction via learned rubrics with a detailed breakdown.

==> fig/bing_result.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for  Microsoft Copilot (Bing
Chat) (Macro)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tiny}
\begin{tabular}{lllllllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$0.4\%$} & \multicolumn{4}{c}{$0.8\%$} & \multicolumn{4}{c}{$2\%$} & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}\cmidrule(l{0.5em}r{0.5em}){18-21}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 77.4 & 73.6 & 74.9 & 74.1 & 77.4 & 73.6 & 74.9 & 74.1 & 77.4 & 73.6 & 74.9 & 74.1 & 77.4 & 73.6 & 74.9 & 74.1 & 77.4 & 73.6 & 74.9 & 74.1\\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
Intruct-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\hline
LinReg-ada-002 & 65.6 & 58.1 & 57.3 & 57.5 & 66.5 & 61.0 & 61.4 & 61.2 & 63.4 & 59.1 & 60.0 & 59.2 & 69.1 & 64.7 & 65.9 & 65.1 & 80.5 & 77.6 & 74.5 & 75.7 \\ 
LogReg-ada-002 & 69.5 & 34.8 & 50.0 & 41.0 & 69.6 & 84.8 & 50.1 & 41.3 & 70.2 & 84.3 & 51.2 & 43.5 & 73.1 & 77.7 & 56.8 & 54.5 & 76.8 & 78.2 & 64.2 & 65.4 \\ 
ASAP & 69.5 & 34.8 & 50.0 & 41.0 & 69.5 & 34.8 & 50.0 & 41.0 & 74.5 & 78.4 & 59.4 & 58.6 & 80.0 & 78.1 & 72.2 & 74.0 & 81.0 & 78.3 & 75.3 & 76.4 \\
USDA & 69.5 & 34.8 & 50.0 & 41.0 & 69.5 & 34.8 & 50.0 & 41.0 & 69.6 & 84.8 & 50.2 & 41.4 & 80.1 & 88.9 & 67.4 & 69.6 & 80.7 & 88.8 & 68.5 & 70.9 \\
\hline
SESRP (Label) & 75.9 & 71.5 & 71.1 & 71.3 & 77.4 & 73.6 & 70.2 & 71.4 & 76.6 & 72.3 & 71.3 & 71.7 & 77.7 & 73.9 & 71.0 & 72.1 & 77.4 & 73.4 & 71.8 & 72.4\\
SESRP (SATv5) & 77.7 & 74.3 & 70.0 & 71.4 & 77.6 & 75.2 & 68.4 & 70.0 & 77.3 & 73.5 & 70.6 & 71.7 & 78.0 & 75.3 & 69.4 & 71.0 & 78.0 & 74.5 & 70.8 & 72.0\\
SESRP-LinReg-ada-002 & 70.7 & 64.8 & 63.6 & 64.0 & 70.4 & 65.4 & 65.7 & 65.5 & 66.6 & 62.2 & 63.4 & 62.5 & 71.9 & 67.6 & 68.9 & 68.1 & 83.4 & 81.2 & 78.2 & 79.4 \\ 
SESRP-LogReg-ada-002 & 69.6 & 81.9 & 50.2 & 41.4 & 72.6 & 80.7 & 55.5 & 51.9 & 77.3 & 79.0 & 64.9 & 66.3 & 79.7 & 78.8 & 70.4 & 72.5 & 81.1 & 79.8 & 73.2 & 75.2 \\ 

\hline
\end{tabular}
\label{tab:task-oriented}
\end{tiny}
\end{center}
\end{table*}


\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for  Microsoft Copilot (Bing
Chat) (weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tiny}
\begin{tabular}{lllllllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$0.4\%$} & \multicolumn{4}{c}{$0.8\%$} & \multicolumn{4}{c}{$2\%$} & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}\cmidrule(l{0.5em}r{0.5em}){18-21}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 77.4 & 78.2 & 77.4 & 77.8 & 77.4 & 78.2 & 77.4 & 77.8 & 77.4 & 78.2 & 77.4 & 77.8 & 77.4 & 78.2 & 77.4 & 77.8 & 77.4 & 78.2 & 77.4 & 77.8\\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
Intruct-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0\\
\hline
LinReg-ada-002 & 65.6 & 64.2 & 65.6 & 64.8 & 66.5 & 67.1 & 66.5 & 66.8 & 63.4 & 65.8 & 63.4 & 64.3 & 69.1 & 70.7 & 69.1 & 69.7 & 80.5 & 79.9 & 80.5 & 79.9 \\ 
LogReg-ada-002 & 69.5 & 48.3 & 69.5 & 57.0 & 69.6 & 78.9 & 69.6 & 57.2 & 70.2 & 78.7 & 70.2 & 58.7 & 73.1 & 75.7 & 73.1 & 65.9 & 76.8 & 77.5 & 76.8 & 73.2 \\ 
ASAP & 69.5 & 48.3 & 69.5 & 57.0 & 69.5 & 48.3 & 69.5 & 57.0 & 74.5 & 76.6 & 74.5 & 68.6 & 80.0 & 79.4 & 80.0 & 78.9 & 81.0 & 80.5 & 81.0 & 80.5\\
USDA & 69.5 & 48.3 & 69.5 & 57.0 & 69.5 & 48.3 & 69.5 & 57.0 & 69.6 & 78.9 & 69.6 & 57.3 & 80.1 & 84.5 & 80.1 & 76.6 & 80.7 & 84.7 & 80.7 & 77.5\\
\hline
SESRP (Label) & 75.9 & 75.7 & 75.9 & \textbf{75.8} & 77.4 & 76.4 & 77.4 & \textbf{76.5} & 76.6 & 76.1 & 76.6 & \textbf{76.3} & 77.7 & 76.8 & 77.7 & \textbf{76.9} & 77.4 & 76.8 & 77.4 & \textbf{77.0}\\
SESRP (SATv5) & 77.7 & 76.7 & 77.7 & \textbf{76.6} & 77.6 & 76.8 & 77.6 & \textbf{75.9} & 77.3 & 76.5 & 77.3 & \textbf{76.6} & 78.0 & 77.1 & 78.0 & \textbf{76.6} & 78.0 & 77.0 & 78.0 & \textbf{77.1} \\% sorry jay I shortent your model names to show the last few columns
SESRP-Lin-ada & 70.7 & 69.7 & 70.7 & 70.1 & 70.4 & 70.8 & 70.4 & 70.6 & 66.6 & 68.6 & 66.6 & 67.4 & 71.9 & 73.2 & 71.9 & 72.4 & 83.4 & 82.9 & 83.4 & 82.9 \\ 
SESRP-Log-ada & 69.6 & 77.1 & 69.6 & 57.3 & 72.6 & 77.3 & 72.6 & 64.2 & 77.3 & 78.1 & 77.3 & 73.8 & 79.7 & 79.3 & 79.7 & 78.0 & 81.1 & 80.7 & 81.1 & 79.9 \\ 

\hline
\end{tabular}
\label{tab:task-oriented}
\end{tiny}
\end{center}
\end{table*}

==> fig/data_stats.tex <==
\begin{table}[htbp]
\caption{Large Data. Train Size: $0.8\%$; Test Size: $80\%$. For learning curve: $0.8\%$, $4\%$, $10\%$, $20\%$; Test Size: $80\%$}
\begin{center}
\begin{tabular}{lll}
\hline
Dataset  & JDDC & Bing \\
\hline
Num. Conversations & 14,389 & 49,998\\
Train  & 128 & 400 \\
Test & 12,854 & 9,998 \\
\hline
\end{tabular}
\label{tab:train_test_0.8}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Small Data. Train Size: $5\%$; Test Size: $60\%$. For learning curve: $5\%$, $10\%$, $20\%$, $40\%$; Test Size: $60\%$}
\begin{center}
\begin{tabular}{llll}
\hline
Dataset  & MWOZ & SGD & Redial \\
\hline
Num. Conversations & 1,155 & 1,683 & 1387  \\
Train & 85 & 121 & 98  \\
Test & 1,375 & 1,943 & 1,571 \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}

==> fig/exp1_topk_precision.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE in the few shot setting.}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{p{4em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}p{1.2em}}
\hline
\multirow{2}{*}{Models} & \multicolumn{4}{c}{Copilot ($0.8\%$)} & \multicolumn{4}{c}{MWOZ ($5\%$)} & \multicolumn{4}{c}{SGD ($5\%$)}  & \multicolumn{4}{c}{ReDial ($5\%$)}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\

\hline
Lin-ada & 66.5 & 67.1 & 66.5 & 66.8 &  27.6 & 44.6 & 27.6 & 31.2 & 38.2 & 53.2 & 38.2 & 42.9 &  28.4 & 48.6 & 28.4 & 33.9 \\
USDA & 69.5 & 48.3 & 69.5 & 57.0 & 47.8 & 22.9 & 47.8 & 30.9 & 70.6 & 68.3 & 70.6 & 64.9 & 38.6 & 70.0 & 38.6 & 24.0 \\
ASAP & 69.5 & 48.3 & 69.5 & 57.0 & 57.1 & 57.9 & 57.1 & 56.9 & 65.8 & 67.3 & 65.8 & 66.4 & 70.2 & 69.5 & 70.2 & 67.6 \\
\hline
Reward & 34.6 & 11.9 & 34.6 & 17.8 & 48.5 & 23.5 & 48.5 & 31.7 & 61.9 & 38.3 & 61.9 & 47.3 & 58.1 & 33.7 & 58.1 & 42.6 \\
ZeroShot & 76.6 & 75.7 & 76.6 & 74.1 & 57.3 & 70.4 & 57.3 & 61.7 & 75.2 & 76.9 & 75.2 & \textbf{75.6} & 63.2 & 40.0 & 63.2 & 49.0 \\
FewShot & 69.4 & 57.9 & 69.4 & 57.2  & 50.0 & 65.6 & 50.0 & 44.2 & 68.2 & 46.8 & 68.2 & 55.5 &  62.2 & 40.0 & 62.2 & 48.7  \\
%Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
% SESRP (Label) & 44.6 & 69.7 & 44.6 & 53.6 & 54.5 & 80.5 & 54.5 & 62.5 & 50.2 & 78.0 & 50.2 & \textbf{50.5} & 43.6 & 73.0 & 43.6 & 52.8 \\
SESRP & 87.0 & 69.0 & 87.0 & 69.0 & 55.0 & 55.0 & 55.0 & 55.0 & 57.0 & 63.0 & 57.0 & 63.0 & 72.0 & 61.0 & 72.0 & 61.0 \\
\hline
\end{tabular}
\label{tab:use_fewshot}
\end{center}
\end{table*}

==> fig/exp1_use_task_oriented.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for task-oriented conversational datasets in the few shot setting (Weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{MWOZ ($5\%$)} & \multicolumn{4}{c}{SGD($5\%$)} & \multicolumn{4}{c}{JDDC($0.8\%$)} & \multicolumn{4}{c}{ReDial($5\%$)}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 46.1 & 61.3 & 46.1 & 52.1 & 75.2 & 76.9 & 75.2 & \textbf{75.6} & 9.7 & 60.6 & 9.7 & 16.7 & 63.2 & 40.0 & 63.2 & 49.0 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 48.5 & 23.5 & 48.5 & 31.7 & 61.9 & 38.3 & 61.9 & 47.3 & 34.6 & 11.9 & 34.6 & 17.8 & 58.1 & 33.7 & 58.1 & 42.6 \\
\hline
LinReg-ada-002 &  27.6 & 44.6 & 27.6 & 31.2 & 38.2 & 53.2 & 38.2 & 42.9 &  41.5 & 42.5 & 41.5 & 41.4 & 00.0 & 00.0 & 00.0 & 00.0 \\
LogReg-ada-002 & 44.4 & 19.8 & 44.4 & 27.4 & 28.6 & 8.2 & 28.6 & 12.7 & 26.7 & 29.8 & 26.7 & 13.5 & 00.0 & 00.0 & 00.0 & 00.0 \\
USDA & 47.8 & 22.9 & 47.8 & 30.9 & 70.6 & 68.3 & 70.6 & 64.9 & 13.3 & 59.9 & 13.3 & 18.8 & 38.6 & 70.0 & 38.6 & 24.0 \\
ASAP & 57.1 & 57.9 & 57.1 & 56.9 & 65.8 & 67.3 & 65.8 & 66.4 & 53.8 & 47.3 & 53.8 & 45.2 & 70.2 & 69.5 & 70.2 & 67.6 \\
\hline
% SESRP (Label) & 44.6 & 69.7 & 44.6 & 53.6 & 54.5 & 80.5 & 54.5 & 62.5 & 50.2 & 78.0 & 50.2 & \textbf{50.5} & 43.6 & 73.0 & 43.6 & 52.8 \\
SESRP (Satv5) & 62.7 & 64.3 & 62.7 & \textbf{63.5} & 75.4 & 74.7 & 75.4 & 72.7 & 27.4 & 68.1 & 27.4 & 30.9 & 71.1 & 70.4 & 71.1 & \textbf{70.5} \\
SESRP-LinReg-ada-002 & 26.0 & 49.0 & 26.0 & 30.8 & 45.6 & 45.9 & 39.6 & 39.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
SESRP-LogReg-ada-002 & 44.4 & 19.8 & 44.4 & 27.4 & 28.6 & 8.2 & 28.6 & 12.7 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
\end{tabular}
\label{tab:task-oriented}
\end{center}
\end{table*}


% \begin{table*}[htbp]
% \caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for task-oriented conversational datasets in the few shot setting}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllllllllllllllll}
% \hline
% \multirow{2}{*}{Models}  & \multicolumn{4}{c}{MWOZ} & \multicolumn{4}{c}{SGD} & \multicolumn{4}{c}{JDDC} & \multicolumn{4}{c}{ReDial}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
%   & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
% \hline
% Zero-Shot &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \hline
% ASAP (weighted) & 54.3 & 50.5 & 54.3 & 52.2 & 66.04 & 59.0 & 66.0 & 61.5 & 56.8 & 48.0 & 56.8 & 48.31 & 58.1 & 49.6 & 58.1 & 50.9 \\
% USDA &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% \hline
% LinReg + ada-002 & 28.9 & 14.3 & 11.7 & 10.7 & 27.5 & 14.0 & 9.9 & 10.2 & 35.5 & 12.6 & 10.5 & 11.4 & 26.2 & 13.4 & 11.2 & 9.8 \\
% LogReg + ada-002 & 44.4 & 14.8 & 33.3 & 20.5 & 28.6 & 9.5 & 33.3 & 14.8 & 31.2 & 27.1 & 36.0 & 24.5 & 33.8 & 11.3 & 33.3 & 16.8 \\
% LinReg + E5L & 24.8 & 11.1 & 10.2 & 8.5 & 24.0 & 9.3 & 6.6 & 6.7 & 36.8 & 12.6 & 11.6 & 11.9 & 23.4 & 9.8 & 7.1 & 7.0 \\
% LogReg + E5L & 44.4 & 14.8 & 33.3 & 20.5 & 28.6 & 9.5 & 33.3 & 14.8 & 27.5 & 24.0 & 33.5 & 19.4 & 33.8 & 11.3 & 33.3 &  16.8\\
% \hline
% SESRP (SATv5 weighted) & 54.9 & 53.7 & 54.9 & 53.2 & 62.2 & 59.2 & 62.2 & 60.7 & 31.1 & 44.7 & 31.1 & 26.6 & 39.0 & 55.3 & 39.0 & 39.1 \\
% SESRP (Label weighted) & 55.3 & 51.8 & 55.3 & 50.6 & 68.3 & 61.6 & 68.3 & 63.3 & 37.4 & 27.9 & 37.4 & 28.5 & 50.8 & 56.8 & 50.8 & 47.7 \\
% \hline
% \end{tabular}
% \label{tab:task-oriented}
% \end{center}
% \end{table*}

==> fig/exp5_gpt_improvement.tex <==
\begin{table}[htbp]
\caption{Improvement of GPT Models}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllll}
\hline
Models  & Acc & P & R & F1\\
\hline
SESRP(GPT4) & 78.4 & 77.5 & 78.4 & 77.4  \\
ZeroShot(GPT4)  & 76.6 & 75.7 & 76.6 & 74.1  \\
SESRP(GPT3.5) & 73.9 & 72.5 & 73.9 & 70.3 \\
ZeroShot(GPT3.5)  & 67.5 & 66.1 & 67.5 & 66.6 \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}

==> fig/exp6_use_general_purpose.tex <==

\begin{table}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for  Microsoft Copilot (Bing
Chat)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllllllll}
\hline
\multirow{2}{*}{Models} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}
  & Acc & P & R & F1 & \\
\hline
ZeroShot & 76.8 & 77.9 & 76.8 & 77.2 \\
\hline
LinReg-ada & 80.5 & 79.9 & 80.5 & 79.9 \\ 
LogReg-ada & 76.8 & 77.5 & 76.8 & 73.2 \\ 
ASAP & 81.0 & 80.5 & 81.0 & 80.5\\
USDA & 80.7 & 84.7 & 80.7 & 77.5\\
\hline
SESRP-Li-ad & 83.4 & 82.9 & 83.4 & \textbf{82.9} \\ 
SESRP-Lo-ad & 81.1 & 80.7 & 81.1 & 79.9 \\ 
\hline
\end{tabular}
\label{tab:copilot}
\end{center}
\end{table}


% \begin{table*}[htbp]
% \caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for  Microsoft Copilot (Bing
% Chat) datasets in the few shot setting}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllllllllllllllll}
% \hline
% \multirow{2}{*}{Models}  & \multicolumn{4}{c}{$0.8\%$} & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
%   & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
% \hline
% Zero-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% \hline
% ASAP (binary-sat) & 69.5 & 69.5 & 100.0 & 82.0 & 80.04 & 81.5 & 92.3 & 86.6 &  81.5 & 81.2 & 95.4 & 87.7 & 00.0 & 00.0 & 00.0 & 00.0 \\
% ASAP (macro) & 70.9 & 64.4 & 61.2 & 61.8 & 79.6 & 76.8 & 72.6 & 74.0 & 80.9 & 78.7 & 74.0 & 75.6 & 00.0 & 00.0 & 00.0 & 00.0 \\
% \hline
% LinReg-E5L & 51.9 & 71.9 & 67.4 & 69.6 & 60.0 & 73.2 & 71.4 & 72.3  & 67.0 & 74.1 & 81.2 & 77.5 & 70.5 & 74.3 & 87.9 & 80.6 \\
% LinReg-ada-002 & 63.4 & 76.7 & 74.3 & 75.5 & 62.0 & 80.0 & 74.1 & 77.0 & 75.8 & 82.9 & 84.7 & 83.8 & 80.1 & 83.4 & 89.3 & 86.5 \\
% LogReg-E5L & 69.5 & 69.5 & 100.0 & 82.0 & 69.8 & 69.1 & 100.0 & 81.1 & 71.0 & 70.8 & 99.2 & 82.6 & 72.0 & 71.8 & 98.3 & 83.0 \\
% LogReg-ada-002 & 69.6 & 69.6 & 100.0 & 82.1 & 73.1 & 72.6 & 98.6 & 83.6 &  75.1 & 74.7 & 97.1 & 84.5 & 76.8 & 76.4 & 96.5 & 85.3 \\
% \hline
% SESRP (Label-binary-sat) & 77.4 & 80.8 & 88.5 & 84.5 & 77.6 & 81.3 & 88.0 & 84.5 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP (SATv5-binary-sat) & 72.6 & 71.9 & 99.4 & 83.5 & 79.7 & 80.2 & 94.0 & 86.5 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP (Label-macro) & 77.4 & 73.6 & 70.2 & 71.4 & 77.6 & 73.8 & 71.0 & 72.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP (SATv5-macro) & 77.6 & 75.2 & 68.4 & 70.0 & 77.9 & 75.2 & 69.3 & 70.9 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP (Label-weighted) & 77.4 & 76.4 & 77.4 & 76.5 & 77.6 & 76.8 & 77.6 & 76.9 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP (SATv5-weighted) & 77.6 & 76.7 & 77.6 & 75.9 & 77.9 & 77.0 & 77.9 & 76.5 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% \hline
% SESRP-LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP-LinReg-ada-002 & 67.8 & 79.3 & 77.7 & 78.5 & 65.0 & 81.9 & 76.5 & 79.1  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP-LogReg-E5L & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% SESRP-LogReg-ada-002 & 72.6 & 71.9 & 99.4 & 83.4 & 80.0 & 80.1 & 94.0 & 86.5  & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
% \hline
% \end{tabular}
% \label{tab:task-oriented}
% \end{center}
% \end{table*}


% \begin{table}[htbp]
% \caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: $10\%$, Test Size: 40K (Jay Updated)}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllll}
% \hline
% Models  & Acc & P & R & F1\\
% \hline
% ASAP & 00.0 & 00.0 & 00.0 & 00.0  \\
% LinReg-E5L & 67.0 & 74.1 & 81.2 & 77.5  \\
% LinReg-ada-002 & 75.8 & 82.9 & 84.7 & 83.8   \\
% LogReg-E5L & 71.0 & 70.8 & 99.2 & 82.6  \\
% LogReg-ada-002 & 75.1 & 74.7 & 97.1 & 84.5   \\
% \hline
% \end{tabular}
% \label{tab:general_purpose_20k}
% \end{center}
% \end{table}


% \begin{table}[htbp]
% \caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: 0.8\%, Test Size: 40K}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllll}
% \hline
% Models  & Acc & P & R & F1\\
% \hline
% ASAP & 70.9 & 64.4 & 61.2 & 61.8  \\
% LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
% LinReg-ada-002 & 65.0 & 73.7 & 78.6 & 76.1   \\
% LogReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
% LogReg-ada-002 & 0.0 & 0.0 & 0.0 & 0.0   \\
% \hline
% SESRP & 77.4 & 73.6 & 70.2 & 71.4   \\
% \hline
% \end{tabular}
% \label{tab:general_purpose_20k}
% \end{center}
% \end{table}

% \begin{table}[htbp]
% \caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: $5\%$, Test Size: 40K (Jay Updated)}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllll}
% \hline
% Models  & Acc & P & R & F1\\
% \hline
% ASAP & 70.9 & 64.4 & 61.2 & 61.8  \\
% LinReg-E5L & 60.0 & 73.2 & 71.4 & 72.3  \\
% LinReg-ada-002 & 62.0 & 80.0 & 74.1 & 77.0   \\
% LogReg-E5L & 69.8 & 69.1 & 100.0 & 81.1  \\
% LogReg-ada-002 & 73.1 & 72.6 & 98.6 & 83.6   \\
% \hline
% \end{tabular}
% \label{tab:general_purpose_20k}
% \end{center}
% \end{table}





% \begin{table}[htbp]
% \caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: $20\%$, Test Size: 40K (Jay Updated)}
% \vspace{-4mm}
% % \setlength{\tabcolsep}{2.3pt}
% \begin{center}
% \begin{tabular}{lllll}
% \hline
% Models  & Acc & P & R & F1\\
% \hline
% ASAP & 00.0 & 00.0 & 00.0 & 00.0  \\
% LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
% LinReg-ada-002 & 80.1 & 83.4 & 89.3 & 86.5   \\
% LogReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
% LogReg-ada-002 & 0.0 & 0.0 & 0.0 & 0.0   \\
% \hline
% \end{tabular}
% \label{tab:general_purpose_20k}
% \end{center}
% \end{table}





\begin{table}[htbp]
\caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: 400, Test Size: 10K}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllll}
\hline
Models  & Acc & P & R & F1\\
\hline
ASAP & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-ada-002 & 63.0 & 75.9 & 74.5 & 75.2   \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}


\begin{table}[htbp]
\caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: 10K, Test Size: 10K}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllll}
\hline
Models  & Acc & P & R & F1\\
\hline
ASAP & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-ada-002 & 00.0 & 00.0 & 00.0 & 00.0  \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}


\begin{table}[htbp]
\caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: 40K, Test Size: 10K}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllll}
\hline
Models  & Acc & P & R & F1\\
\hline
ASAP & 83.9 & 83.5 & 83.9 & 83.4  \\
LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-ada-002 & 82.5 & 83.4 & 93.7 & 88.2  \\
SESRP-LinReg-ada & 84.8 & 85.7 & 94.0 &  89.7 \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}

\begin{table}[htbp]
\caption{Performance on USE for Microsoft Copilot (Bing Chat). Training Size: 90K, Test Size: 10K}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllll}
\hline
Models  & Acc & P & R & F1\\
\hline
ASAP & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-E5L & 00.0 & 00.0 & 00.0 & 00.0  \\
LinReg-ada-002 & 83.2 & 83.6 & 94.6 & 88.8  \\
SESRP-LinReg-ada & 84.7 & 85.3 & 94.6 & 89.7 \\
\hline
\end{tabular}
\label{tab:general_purpose_20k}
\end{center}
\end{table}





==> fig/exp7_scale.tex <==


\begin{table}[htbp]
\caption{Performance on USE for Microsoft Copilot for different training set sizes for a 10K test set}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{llllll}
\hline
Models  & Train  & Acc & P & R & F1\\
  &  Set &  &  &  & \\
\hline
SESRP & 400 & 78.4 & 77.5 & 78.4 & 77.4 \\
%\hline
%ASAP & 10K & 00.0 & 00.0 & 00.0 & 00.0  \\
%Lin-ada & 10K & 00.0 & 00.0 & 00.0 & 00.0  \\
%SESRP- & 10K & 00.0 & 00.0 & 00.0 & 00.0  \\
%Lin-ada &  &  &  &  &   \\
\hline
ASAP & 40K & 83.9 & 83.5 & 83.9 & 83.4  \\
Lin-ada & 40K & 82.5 & 83.4 & 93.7 & 88.2  \\
SESRP- & 40K & 84.8 & 85.7 & 94.0 &  \textbf{89.7} \\
Lin-ada &  &  &  &  &   \\
Log-ada & 40K & 80.0 & 79.4 & 96.0 & 86.9  \\
SESRP- & 40K & 81.9 & 82.9 & 93.1 & 87.7  \\
Log-ada &  &  &  &  &   \\
\hline
ASAP & 90K & 83.9 & 83.6 & 83.9 & 83.4 \\
Lin-ada & 90K & 83.2 & 83.6 & 94.6 & 88.8  \\
SESRP- & 90K & 84.7 & 85.3 & 94.6 & \textbf{89.7} \\
Lin-ada &  &  &  &  &  \\
Log-ada & 90K & 81.4 & 81.1 & 95.4 & 87.6  \\
SESRP- & 90K & 83.0 & 83.6 & 94.0 & 88.5 \\
Log-ada &  &  &  &  &  \\
\hline
\end{tabular}
\label{tab:general_purpose_scale}
\end{center}
\end{table}



==> fig/jddc_result.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for JDDC (Macro)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllllllll}
\hline
\multirow{2}{*}{Models}   & \multicolumn{4}{c}{$0.8\%$} & \multicolumn{4}{c}{$2\%$} & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 9.7 & 36.4 & 5.8 & 10.0 & 9.7 & 36.4 & 5.8 & 10.0 & 9.7 & 36.4 & 5.8 & 10.0 & 9.7 & 36.4 & 5.8 & 10.0 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Intruct-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 41.5 & 41.8 & 40.4 & 40.6 & 40.0 & 40.5 & 40.4 & 40.1 & 39.1 & 39.4 & 40.2 & 39.0 & 44.1 & 43.7 & 44.1 & 43.9 \\ 
LogReg-ada-002 & 26.7 & 28.0 & 33.9 & 16.1 & 26.6 & 27.9 & 34.0 & 15.7 & 26.2 & 25.2 & 33.5 & 15.1 & 31.2 & 27.1 & 36.0 & 24.5 \\ 
USDA & 13.3 & 40.5 & 7.8 & 11.0 & 39.8 & 49.8 & 23.5 & 27.5 & 67.8 & 55.7 & 44.5 & 49.4 & 76.8 & 58.3 & 50.4 & 53.9 \\
ASAP & 53.8 & 43.2 & 47.1 & 40.4 & 63.2 & 64.7 & 59.5 & 59.6 & 66.7 & 70.7 & 62.4 & 62.3 & 67.8 & 67.6 & 66.3 & 66.7 \\
\hline
SESRP (Label) & 50.2 & 50.3 & 36.6 & 35.3 & 57.2 & 50.0 & 40.6 & 40.3 & 51.9 & 50.4 & 37.5 & 37.4 & 47.7 & 50.7 & 35.3 & 33.3 \\
SESRP (SATv5) & 27.4 & 42.3 & 19.7 & 21.1 & 38.7 & 43.2 & 26.5 & 29.9 & 43.4 & 44.6 & 30.6 & 31.5 & 30.5 & 42.8 & 21.8 & 23.1 \\
SESRP-LinReg-ada-002 & 43.3 & 45.1 & 43.5 & 43.3 & 43.0 & 43.7 & 43.9 & 43.3 & 39.7 & 40.0 & 40.8 & 39.5 & 44.7 & 44.4 & 44.8 & 44.6 \\ 
SESRP-LogReg-ada-002 & 26.7 & 26.8 & 33.8 & 16.5 & 27.5 & 27.9 & 34.3 & 18.1 & 28.0 & 29.2 & 34.7 & 18.7 & 34.4 & 28.3 & 38.0 & 28.1 \\ 
\hline
\end{tabular}
\label{tab:task-oriented}
\end{center}
\end{table*}

\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for JDDC (Weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllllllll}
\hline
\multirow{2}{*}{Models}   & \multicolumn{4}{c}{$0.8\%$} & \multicolumn{4}{c}{$2\%$} & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$20\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 9.7 & 60.6 & 9.7 & 16.7 & 9.7 & 60.6 & 9.7 & 16.7 & 9.7 & 60.6 & 9.7 & 16.7 & 9.7 & 60.6 & 9.7 & 16.7 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Intruct-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 41.5 & 42.5 & 41.5 & 41.4 & 40.0 & 41.1 & 40.0 & 40.3 & 39.1 & 40.2 & 39.1 & 38.9 & 44.1 & 44.2 & 44.1 & 44.1 \\ 
LogReg-ada-002 & 26.7 & 29.8 & 26.7 & 13.5 & 26.6 & 29.6 & 26.6 & 12.9 & 26.2 & 26.4 & 26.2 & 12.3 & 31.2 & 28.7 & 31.2 & 23.7 \\ 
USDA & 13.3 & 59.9 & 13.3 & 18.8 & 39.8 & 76.0 & 39.8 & 46.0 & 67.8 & 84.4 & 67.8 & 75.2 & 76.8 & 87.5 & 76.8 & 81.6 \\
ASAP & 53.8 & 47.3 & 53.8 & 45.2 & 63.2 & 64.6 & 63.2 & 61.6 & 66.7 & 70.1 & 66.7 & 64.6 & 67.8 & 68.0 & 67.8 & 67.7 \\
\hline
SESRP (Label) & 50.2 & 78.0 & 50.2 & \textbf{50.5} & 57.2 & 77.4 & 57.2 & \textbf{59.0} & 51.9 & 77.9 & 51.9 & \textbf{54.0} & 47.7 & 78.7 & 47.7 & \textbf{47.0} \\
SESRP (SATv5) & 27.4 & 68.1 & 27.4 & \textbf{30.9} & 38.7 & 68.8 & 38.7 & \textbf{45.3} & 43.4 & 70.6 & 43.4 & \textbf{46.9} & 30.5 & 68.6 & 30.5 & \textbf{33.9} \\
SESRP-LinReg-ada-002-SAT & 43.3 & 45.6 & 43.3 & 43.5 & 43.0 & 44.3 & 43.0 & 43.2 & 39.7 & 40.7 & 39.7 & 39.4 & 44.7 & 44.9 & 44.7 & 44.7 \\ 
SESRP-LogReg-ada-002-SAT & 26.7 & 28.3 & 26.7 & 14.0 & 27.5 & 29.7 & 27.5 & 15.9 & 28.0 & 31.2 & 28.0 & 16.5 & 34.4 & 30.0 & 34.4 & 28.0 \\ 
\hline
\end{tabular}
\label{tab:task-oriented}
\end{center}
\end{table*}


==> fig/mwoz_result.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for MWOZ (macro)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 46.1 & 40.6 & 30.3 & 34.3 & 46.1 & 40.6 & 30.3 & 34.3 & 46.1 & 40.6 & 30.3 & 34.3 & 46.1 & 40.6 & 30.3 & 34.3 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 27.6 & 34.1 & 35.5 & 26.4 & 27.1 & 34.6 & 32.3 & 26.1 & 35.1 & 36.8 & 35.7 & 31.6 & 36.9 & 37.3 & 37.6 & 33.0 \\ 
LogReg-ada-002 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 \\ 
USDA& 47.8 & 23.9 & 50.0 & 32.4 & 49.5 & 59.5 & 51.5 & 37.7 & 52.2 & 26.1 & 50.0 & 34.3 & 52.2 & 51.1 & 50.0 & 34.9 \\
ASAP & 57.1 & 57.7 & 57.5 & 57.0 & 57.6 & 57.5 & 57.3 & 57.3 & 59.0 & 59.7 & 59.4 & 58.8 & 62.0 & 61.9 & 61.7 & 61.7 \\
\hline
SESRP (Label) & 44.6 & 46.5 & 29.4 & \textbf{35.5} & 42.2 & 46.6 & 27.8 & \textbf{34.4} & 38.4 & 48.7 & 25.1 & \textbf{31.9} & 50.0 & 44.6 & 32.6 & \textbf{34.4} \\
SESRP (Satv5) & 62.7 & 42.8 & 41.8 & \textbf{42.3} & 55.7 & 42.0 & 37.4 & \textbf{38.9} & 61.2 & 43.2 & 41.3 & \textbf{40.6 }& 62.6 & 42.9 & 41.3 & \textbf{41.6} \\
SESRP-LinReg-ada-002 & 26.0 & 36.9 & 33.7 & 25.5 & 30.6 & 38.0 & 37.5 & 29.4 & 37.4 & 39.6 & 37.9 & 33.7 & 36.5 & 37.0 & 36.8 & 32.6 \\ 
SESRP-LogReg-ada-002 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 & 44.4 & 14.8 & 33.3 & 20.5 \\ 
\hline
\end{tabular}
\label{tab:mwoz_macro}
\end{center}
\end{table*}


\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for MWOZ (weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 46.1 & 61.3 & 46.1 & 52.1 & 46.1 & 61.3 & 46.1 & 52.1 & 46.1 & 61.3 & 46.1 & 52.1 & 46.1 & 61.3 & 46.1 & 52.1 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 27.6 & 44.6 & 27.6 & 31.2 & 27.1 & 45.7 & 27.1 & 31.8 & 35.1 & 48.6 & 35.1 & 39.3 & 36.9 & 48.9 & 36.9 & 40.5 \\ 
LogReg-ada-002 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 \\ 
USDA& 47.8 & 22.9 & 47.8 & 30.9 & 49.5 & 60.0 & 49.5 & 36.5 & 52.2 & 27.2 & 52.2 & 35.8 & 52.2 & 51.1 & 52.2 & 36.3 \\
ASAP & 57.1 & 57.9 & 57.1 & 56.9 & 57.6 & 57.5 & 57.6 & 57.5 & 59.0 & 59.9 & 59.0 & 58.7 & 62.0 & 61.9 & 62.0 & 61.8 \\
\hline
SESRP (Label) & 44.6 & 69.7 & 44.6 & \textbf{53.6} & 42.2 & 69.9 & 42.2 &\textbf{ 52.0} & 38.4 & 73.0 & \textbf{38.4} & 48.5 & 50.0 & 66.7 & 50.0 & \textbf{52.3} \\
SESRP (Satv5) & 62.7 & 64.3 & 62.7 & \textbf{63.5} & 55.7 & 63.3 & 55.7 & \textbf{58.4} & 61.2 & 65.2 & \textbf{61.2} & 60.6 & 62.6 & 64.3 & 62.6 & \textbf{62.7 }\\
SESRP-LinReg-ada-002 & 26.0 & 49.0 & 26.0 & 30.8 & 30.6 & 49.9 & 30.6 & 35.6 & 37.4 & 52.4 & 37.4 & 42.1 & 36.5 & 48.7 & 36.5 & 40.3 \\ 
SESRP-LogReg-ada-002 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 & 44.4 & 19.8 & 44.4 & 27.4 \\  
\hline
\end{tabular}
\label{tab:mwoz_weighted}
\end{center}
\end{table*}

==> fig/redial_result.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for ReDial (macro)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 46.2 & 42.1 & 27.7 & 33.3 & 46.2 & 42.1 & 27.7 & 33.3 & 46.2 & 42.1 & 27.7 & 33.3 & 46.2 & 42.1 & 27.7 & 33.3 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 28.4 & 33.7 & 29.6 & 25.5 & 32.7 & 34.2 & 31.4 & 27.9 & 38.8 & 37.5 & 37.8 & 33.1 & 41.5 & 38.3 & 37.2 & 35.2 \\ 
LogReg-ada-002 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 \\ 
USDA& 38.6 & 63.1 & 51.3 & 30.4 & 63.7 & 58.9 & 55.3 & 53.6 & 62.2 & 56.6 & 54.5 & 53.3 & 68.3 & 68.1 & 59.5 & 58.3 \\
ASAP & 56.3 & 59.6 & 59.8 & 56.3 & 59.2 & 55.0 & 54.6 & 54.6 & 66.1 & 63.7 & 57.0 & 55.2 & 70.2 & 69.0 & 63.2 & 63.4 \\
\hline
SESRP (Label) & 43.6 & 46.4 & 30.6 & 35.6 & 45.8 & 45.8 & 32.6 & 36.3 & 47.3 & 48.5 & 31.4 & 37.9 & 43.5 & 45.8 & 29.6 & 35.5\\
SESRP (Satv5) & 53.1 & 41.9 & 39.5 & 35.6 & 50.3 & 42.3 & 37.4 & 34.4 & 61.1 & 43.4 & 42.3 & 41.2 & 53.5 & 41.9 & 38.2 & 36.9 \\
SESRP-LinReg-ada-002 & 30.8 & 40.6 & 35.3 & 28.9 & 36.5 & 39.0 & 36.4 & 32.0 & 39.7 & 38.8 & 41.2 & 34.7 & 43.8 & 40.6 & 40.1 & 37.2 \\ 
SESRP-LogReg-ada-002 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 & 33.8 & 11.3 & 33.3 & 16.8 \\ 
\hline
\end{tabular}
\label{tab:redial_macro}
\end{center}
\end{table*}


\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for ReDial (weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 46.2 & 68.2 & 46.2 & 54.9 & 46.2 & 68.2 & 46.2 & 54.9 & 46.2 & 68.2 & 46.2 & 54.9 & 46.2 & 68.2 & 46.2 & 54.9 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 28.4 & 48.6 & 28.4 & 33.9 & 32.7 & 47.9 & 32.7 & 37.4 & 38.8 & 50.9 & 38.8 & 42.6 & 41.5 & 52.7 & 41.5 & 45.6 \\ 
LogReg-ada-002 & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 \\ 
USDA& 38.6 & 70.0 & 38.6 & 24.0 & 63.7 & 60.8 & 63.7 & 59.3 & 62.2 & 59.0 & 62.2 & 58.7 & 68.3 & 68.2 & 68.3 & 63.7 \\
ASAP & 56.3 & 63.7 & 56.3 & 56.5 & 59.2 & 58.0 & 59.2 & 58.4 & 66.1 & 64.6 & 66.1 & 61.0 & 70.2 & 69.5 & 70.2 & 67.6 \\
\hline
SESRP (Label) & 43.6 & 73.0 & 43.6 & \textbf{52.8} & 45.8 & 72.3 & 45.8 & \textbf{53.7} & 47.3 & 75.7 & 47.3 & \textbf{58.0} & 43.5 & 71.6 & 43.5 & \textbf{53.5} \\
SESRP (Satv5) & 53.1 & 68.0 & 53.1 & \textbf{52.6} & 50.3 & 69.2 & 50.3 & \textbf{50.9} & 61.1 & 69.6 & 61.1 & \textbf{62.8} & 53.5 & 67.8 & 53.5 & \textbf{55.6} \\
SESRP-LinReg-ada-002-SAT weighted & 30.8 & 57.5 & 30.8 & 37.2 & 36.5 & 54.2 & 36.5 & 42.0 & 39.7 & 52.0 & 39.7 & 43.4 & 43.8 & 55.3 & 43.8 & 47.9 \\ 
SESRP-LogReg-ada-002-SAT weighted & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 & 33.8 & 11.4 & 33.8 & 17.1 \\ 
\hline
\end{tabular}
\label{tab:redial_weighted}
\end{center}
\end{table*}

==> fig/sgd_result.tex <==
\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for SGD (macro)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot &  69.6 & 48.6 & 39.9 & 42.6 &  69.6 & 48.6 & 39.9 & 42.6 & 69.6 & 48.6 & 39.9 & 42.6 &  69.6 & 48.6 & 39.9 & 42.6 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 38.2 & 38.6 & 34.8 & 32.2 & 36.6 & 37.4 & 34.5 & 32.3 & 41.7 & 38.3 & 36.1 & 34.7 & 46.2 & 39.0 & 37.8 & 37.1 \\ 
LogReg-ada-002 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 \\ 
USDA& 70.6 & 66.4 & 56.7 & 55.2 & 57.5 & 62.4 & 63.6 & 57.3 & 70.6 & 64.9 & 60.4 & 60.9 & 73.5 & 70.0 & 71.3 & 70.5 \\
ASAP & 65.8 & 61.7 & 62.6 & 62.0 & 72.8 & 68.1 & 66.0 & 66.7 & 74.7 & 70.7 & 70.4 & 70.5 & 73.2 & 68.9 & 68.6 & 68.7 \\
\hline
SESRP (Label) & 54.7 & 51.3 & 29.9 & 35.6 & 44.2 & 51.5 & 25.8 & 33.6 & 60.3 & 49.8 & 31.7 & 34.0 & 52.6 & 53.7 & 30.1 & 37.3 \\
SESRP (Satv5) & 71.1 & 46.7 & 47.5 & 46.5 & 59.4 & 41.6 & 41.0 & 39.5 & 72.1 & 45.1 & 43.9 & 44.4 & 64.9 & 44.6 & 45.3 & 42.9 \\
SESRP-LinReg-ada-002 & 45.6 & 45.9 & 39.6 & 39.0 & 43.1 & 44.5 & 42.0 & 38.7 & 45.2 & 41.1 & 40.4 & 38.2 & 47.7 & 40.9 & 40.3 & 39.2 \\ 
SESRP-LogReg-ada-002 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 & 28.6 & 9.5 & 33.3 & 14.8 \\ 
\hline
\end{tabular}
\label{tab:sgd_macro}
\end{center}
\end{table*}


\begin{table*}[htbp]
\caption{Accuracy (Acc), Precision (P), Recall (R), and F1 Score (F1) on USE for SGD (weighted)}
\vspace{-4mm}
% \setlength{\tabcolsep}{2.3pt}
\begin{center}
\begin{tabular}{lllllllllllllllll}
\hline
\multirow{2}{*}{Models}  & \multicolumn{4}{c}{$5\%$} & \multicolumn{4}{c}{$10\%$} & \multicolumn{4}{c}{$20\%$} & \multicolumn{4}{c}{$40\%$}\\ \cmidrule(l{0.5em}r{0.5em}){2-5}\cmidrule(l{0.5em}r{0.5em}){6-9}\cmidrule(l{0.5em}r{0.5em}){10-13}\cmidrule(l{0.5em}r{0.5em}){14-17}
  & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1 & Acc & P & R & F1\\
\hline
Zero-Shot & 69.6 & 76.0 & 69.6 & 71.2 & 69.6 & 76.0 & 69.6 & 71.2 &69.6 & 76.0 & 69.6 & 71.2 & 69.6 & 76.0 & 69.6 & 71.2 \\
Few-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Inst-Shot & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
Reward & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\hline
LinReg-ada-002 & 38.2 & 53.2 & 38.2 & 42.9 & 36.6 & 52.1 & 36.6 & 41.7 & 41.7 & 53.8 & 41.7 & 46.1 & 46.2 & 54.5 & 46.2 & 49.6 \\ 
LogReg-ada-002 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 \\ 
USDA& 70.6 & 68.3 & 70.6 & 64.9 & 57.5 & 70.2 & 57.5 & 58.4 & 70.6 & 68.2 & 70.6 & 68.0 & 73.5 & 74.7 & 73.5 & 74.0 \\
ASAP & 65.8 & 67.3 & 65.8 & 66.4 & 72.8 & 71.6 & 72.8 & 71.9 & 74.7 & 74.5 & 74.7 & 74.6 & 73.2 & 73.0 & 73.2 & 73.1 \\
\hline
SESRP (Label) & 54.7 & 80.4 & 54.7 & \textbf{62.5} & 44.2 & 79.9 & 44.2 & \textbf{56.1} & 60.3 & 76.1 & 60.3 & \textbf{61.7} & 52.6 & 82.6 & 52.6 & \textbf{62.7} \\
SESRP (Satv5) & 71.1 & 75.8 & 71.1 & \textbf{72.6} & 59.4 & 69.9 & 59.4 & \textbf{61.9} & 72.1 & 71.5 & 72.1 & \textbf{71.6} & 64.9 & 74.2 & 64.9 & \textbf{66.7} \\
SESRP-LinReg-ada-002 & 45.6 & 61.0 & 45.6 & 51.0 & 43.1 & 60.0 & 43.1 & 48.5 & 45.2 & 56.2 & 45.2 & 49.2 & 47.7 & 55.9 & 47.7 & 51.0 \\ 
SESRP-LogReg-ada-002 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 & 28.6 & 8.2 & 28.6 & 12.7 \\
\hline
\end{tabular}
\label{tab:sgd_weighted}
\end{center}
\end{table*}
